Consolidating Diffusion-Generated Video Detection with Unified Multimodal Forgery Learning

The proliferation of videos generated by diffusion models has raised increasing concerns about information security, highlighting the urgent need for reliable detection of synthetic media. Existing methods primarily focus on image-level forgery detection, leaving generic video-level forgery detection largely underexplored. To advance video forensics, we propose a consolidated multimodal detection algorithm, named MM-Det++, specifically designed for detecting diffusion-generated videos. Our approach consists of two innovative branches and a Unified Multimodal Learning (UML) module. Specifically, the Spatio-Temporal (ST) branch employs a novel Frame-Centric Vision Transformer (FC-ViT) to aggregate spatio-temporal information for detecting diffusion-generated videos, where the FC-tokens enable the capture of holistic forgery traces from each video frame. In parallel, the Multimodal (MM) branch adopts a learnable reasoning paradigm to acquire Multimodal Forgery Representation (MFR) by harnessing the powerful comprehension and reasoning capabilities of Multimodal Large Language Models (MLLMs), which discerns the forgery traces from a flexible semantic perspective. To integrate multimodal representations into a coherent space, a UML module is introduced to consolidate the generalization ability of MM-Det++. In addition, we also establish a large-scale and comprehensive Diffusion Video Forensics (DVF) dataset to advance research in video forgery detection. Extensive experiments demonstrate the superiority of MM-Det++ and highlight the effectiveness of unified multimodal forgery learning in detecting diffusion-generated videos.

==> figs/architecture_figure.tex <==
\begin{figure}[tb]
  \centering
  \includesvg[width=\linewidth]{figs/overview_of_main_method.svg}
  \caption{The framework of Multi-Modal Detection (MM-Det): 
  % The model learns multimodal forgery invariant representation in the LMM branch and captures spatial-temporal artifacts in the ST branch. 
  Given an input video, the language multi-modal model takes the frame and instructions to generate the response. Hidden states from the vision encoder and transformer decoder are extracted to form a multi-modal representation, denoted as $\mathbf{F}_{M}$, which helps capture the forgery traces among different diffusion-generated videos. In the spatial-temporal branch, videos are fed into a CNN encoder, followed by a Transformer-based network to model sequential information. An In-and-Across Frame Attention(IAFA) module is introduced to capture frame-level spatial artifacts and temporal inconsistencies, termed as $\mathbf{F}_{ST}$. At last, a well-designed dynamic fusion strategy combines $\mathbf{F}_{M}$ and $\mathbf{F}_{ST}$ for the effective video forgery prediction. \vspace{-3mm}}
  \label{fig:overview_of_main_model}
\end{figure}

==> latex_table_figures/exp_detection_frame.tex <==

\begin{table}[t]
  \caption{Frame-level forgery detection performance, which averages 15 forgery methods including GAN and diffusion.}
  \label{tab:frame_dataset_evaluation}
  \centering
  \resizebox{0.98\linewidth}{!}{

  \begin{tabular}{c|cc|c}
     \hline
    % \multirow{2}{*}{Method} & \multirow{2}{*}{{\makecellTraining Dataset} & \multirow{2}{*}{Generative Type} & \multirow{2}{*}{Detection Level} & \multicolumn{2}{c}{SVD} & \multicolumn{2}{c}{VideoCrafter} & \multicolumn{2}{c}{Zeroscope} & \multicolumn{2}{c}{Diffusion Roop} & \multicolumn{2}{c}{Avg} \\
    \multirow{2}{*}{Method}&GAN-based & Diffusion-based & Avg \\
    \cline{2-4}
    &\multicolumn{3}{c}{\textit{Metric:} AUC (\%)} \\
    \hline
    Universal FD & $\mathbf{95.8}$ & $\mathbf{95.6}$ & $\mathbf{95.7}$\\
    \hline
    Ours & $\mathbf{95.8}$ & $95.2$ & $95.5$\\
  \hline
  \end{tabular}
  }
\end{table}

==> latex_table_figures/exp_detection_frame_extension.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/pdfs/expt_frame_level_extension.pdf}
    \caption{We append multiple sequential decoders (\textit{e.g.}, LSTM, ViT, ViViT and FC-ViT) at the end of existing frame-level detection methods for an extension on video-level prediction.
    % For frame-level detectors, we extend them to video detection by appending a decoder after the encoding stage. Frame-level features from the latent space are extracted as the input of the decoder, which predicts a binary class for each video clip.
    }
    \label{fig:expt_frame_level_extension}
\end{figure}

==> latex_table_figures/figure_text_image_pair_dataset.tex <==
\begin{figure}[tb]

\centering
\includegraphics[width=0.96\linewidth]{figs/pdfs/text-image_dataset.pdf}
\caption{Rich Forgery Reasoning Dataset. We rely on Gemini's inference ability for high-quality descriptions. Instructions are sampled from the pre-defined template for guidance in analyzing and reasoning about authenticity. The reasons and inference results are processed to form the forgery description for each frame and serve as the dataset for LMM finetuning.}
\label{fig:text_image_pair_dataset}
\end{figure}
